Make Your Brief Stroke Real and Stereoscopic: 3D-Aware Simplified Sketch to Portrait Generation

Creating the photo-realistic version of people sketched portraits is useful to various entertainment purposes. Existing studies only generate portraits in the 2D plane with fixed views, making the results less vivid. In this paper, we present Stereoscopic Simplified Sketch-to-Portrait (SSSP), which explores the possibility of creating Stereoscopic 3D-aware portraits from simple contour sketches by involving 3D generative models. Our key insight is to design sketch-aware constraints that can fully exploit the prior knowledge of a tri-plane-based 3D-aware generative model. Specifically, our designed region-aware volume rendering strategy and global consistency constraint further enhance detail correspondences during sketch encoding. Moreover, in order to facilitate the usage of layman users, we propose a Contour-to-Sketch module with vector quantized representations, so that easily drawn contours can directly guide the generation of 3D portraits. Extensive comparisons show that our method generates high-quality results that match the sketch. Our usability study verifies that our system is greatly preferred by user.

==> sections/biography.tex <==

% \vspace{-35pt}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{photos/yasheng_sun.jpg}}]{Yasheng Sun} received the ME degrees from the School of Mechanical Engineering, Shanghai Jiao Tong University, China, in 2020. He is currently pursing the Ph.D. degree in Computer Science from School of Computing, Tokyo Institute of Technology, Japan. His current research interest includes cross-modal generation, 3D generative model and its application in computer vision.
\end{IEEEbiography}

\vspace{-25pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{photos/qianyi_wu.jpeg}}]{Qianyi Wu}
received the BSc and MSc degrees from the Special Class for the Gifted Youth and School of Mathematical Sciences, University of Science and Technology of China in 2016 and 2019, respectively.  He is currently pursuing the Ph.D. degree with the Faculty of Information Technology, the Monash University. His current research interest includes computer vision and computer graphics.
\end{IEEEbiography}

\vspace{-25pt}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{photos/hang_zhou.jpg}}]{Hang Zhou}
is now a researcher at Baidu Inc. He obtained his Ph.D. degree from Multimedia Lab (MMLab), The Chinese University of Hong Kong in 2021, supervised by Prof. Xiaogang Wang. He received his bachelor's degree in Acoustics from the School of Physics at Nanjing University (NJU) in 2017.
\end{IEEEbiography}

\vspace{-25pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{photos/kaisiyuan_wang.jpg}}]{Kaisiyuan Wang}
received the BE and ME degrees from the School of Electrical Engineering, Harbin Institute of Technology, China, in 2016 and 2018, respectively.  He is currently pursuing the Ph.D. degree with the School of Electrical and Information Engineering, the University of Sydney. His current research interest includes 3D low-level vision and its applications in computer vision.
\end{IEEEbiography}

\vspace{-25pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{photos/hutianshu.jpeg}}]{Tianshu Hu}
is now a computer vision researcher at Baidu Inc. He obtained his bachelor degree from University of Stuttgart in 2016 and master degree from ETH Zurich in 2019, respectively.
\end{IEEEbiography}

\vspace{-25pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{photos/liao.png}}]{Chen-Chieh Liao} is a Ph.D. student at the School of Computing, Tokyo Institute of Technology, Japan from 2022. He received his B.E. and M.S. degrees from the Tokyo Institute of Technology in 2020 and 2022. His research interests lie primarily in human-computer interaction, mixed/augmented reality, and machine vision.
\end{IEEEbiography}

\vspace{-25pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{photos/dongliang_he.png}}]{Dongliang He}
received the bachelor’s and the Ph.D. degree in computer science from the University of Science and Technology of China, Hefei, China, in 2012 and 2017, respectively. He is currently a Senior Research and Development Engineer with the Department of Computer Vision Technology, Baidu Inc., Beijing, China. His research interests focus on computer vision, deep learning, and multimedia processing.
\end{IEEEbiography}

\vspace{-25pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{photos/jingtuo_liu.png}}]{Jingtuo Liu}
received the B.S. and M.S. degrees in electronics and engineering from Tsinghua University in 2008 and 2011, respectively. Since 2011, he has been working on computer vision at Baidu, Inc., where he is currently a Chief Architect with the Computer Vision Team. His research interests focus on face detection and recognition and optical character recognition.
\end{IEEEbiography}

\vspace{-25pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{photos/errui_ding.png}}]{Errui Ding}
received the Ph.D. degree from Xidian University, Xi'an, China, in 2008.
He is currently the Director of the Computer Vision Technology Department (VIS) and Augmented Reality Department (AR), Baidu Inc.    
\end{IEEEbiography}

\vspace{-25pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{photos/jingdong_wang.png}}]{Jingdong Wang}(Fellow, IEEE)
is Chief Architect for computer vision with the Artificial Intelligence Group at Baidu.
% His areas of interest include neural architecture design, human pose estimation, semantic segmentation, image classification, object detection, large-scale indexing, and salient object detection. 
He has been serving/served as an Associate Editor of IEEE TPAMI, IJCV, IEEE TMM, and IEEE TCSVT, and an area chair of leading conferences in vision, multimedia, and AI, such as CVPR, ICCV, ECCV, ACM MM, IJCAI, and AAAI. He was elected as an ACM Distinguished Member, a Fellow of IAPR, and a Fellow of IEEE, for his contributions to visual content understanding and retrieval.    
\end{IEEEbiography}

\vspace{-25pt}
% \enlargethispage{-10cm}

% \newpage

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{photos/miyafuji.jpeg}}]{Shio Miyafuji}
is currently a Assistant professor at School of Computing in Tokyo Institute of Technology. Her research interests focus on human-computer interaction, mixed augmented reality and optical projectors.
\end{IEEEbiography}

\vspace{-25pt}

% \enlargethispage{-18cm}

% \newpage


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{photos/ziwei_liu.png}}]{Ziwei Liu}
is a Nanyang Assistant Professor at School of Computer Science and Engineering (SCSE) in Nanyang Technological University, with MMLab@NTU. Previously, he was a research fellow (2018-2020) in CUHK (with Prof. Dahua Lin) and a post-doc researcher (2017-2018) in UC Berkeley (with Prof. Stella X. Yu). His research interests include computer vision, machine learning and computer graphics. He received his Ph.D. (2013-2017) from CUHK / Multimedia Lab.
\end{IEEEbiography}

\vspace{-25pt}
% \enlargethispage{-13cm}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip]{photos/koike.jpeg}}]{Hideki Koike}
received the B.E., M.E., and Dr.Eng. degrees from the University of Tokyo, in 1986, 1988, and 1991, respectively. He was at the University of Electro-Communications, Tokyo. In 2014, he joined Tokyo Institute of Technology, Japan, where he is a Professor with the School of Computing. His research interests include vision-based human–computer interaction, human augmentation, information visualization, and usable security.
\end{IEEEbiography}


% \vspace{-250pt}

